Genuine Personal Identifiers and Mutual Sureties for Sybil-Resilient Community Formation

While most of humanity is suddenly on the net, the value of this singularity is hampered by the lack of credible digital identities: Social networking, person-to-person transactions, democratic conduct, cooperation and philanthropy are all hampered by the profound presence of fake identities, as illustrated by Facebook's removal of 5.4Bn fake accounts since the beginning of 2019. Here, we introduce the fundamental notion of a \emph{genuine personal identifier}---a globally unique and singular identifier of a person---and present a foundation for a decentralized, grassroots, bottom-up process in which every human being may create, own, and protect the privacy of a genuine personal identifier. The solution employs mutual sureties among owners of personal identifiers, resulting in a mutual-surety graph reminiscent of a web-of-trust. Importantly, this approach is designed for a distributed realization, possibly using distributed ledger technology, and does not depend on the use or storage of biometric properties. For the solution to be complete, additional components are needed, notably a mechanism that encourages honest behavior and a sybil-resilient governance system.

==> backup.tex <==
* Some stuff that got deleted

The following definition formalizes the notion that a global identifier is \emph{genuine} if it has a sole owner that owns no other global identifier.

\begin{definition}[Compromised, Duplicated, Sybil and Genuine Global Identifiers]
Let $V$ be a set of global identifiers. A global identifier $v \in V$ is  \emph{compromised} in $V$ if it has more than one owner in $V$ and \emph{duplicated} in $V$ if it has an owner that owns another global identifier $v'\ne v \in V$, in which case $v$ and $v'$ are \emph{duplicates}. A global identifier that is compromised or duplicated in is a \emph{sybil}, else \emph{genuine}, all relative to $V$.
\end{definition}

That is, a genuine global identity is neither compromised (with multiple owners) nor duplicated (with an owner that owns additional global identifiers).  Note that a compromised global identity would typically also be duplicated, since its spurious owners, to be effective in their ploy, will have to own additional global identifiers.


Note that:
\begin{itemize}
    \item An owner of a global identity $v \in V$ knows an owner of $v' \in V$ if $own_h(v) \in \calK$ and $K_h own_{h'}(v') \in \calK$ for some $h, h' \in \calH$ and some $s$.  
    \item An agent $h \in \calH$ knows that a global identity $v' \in V$ is compromised if $h$ knows two distinct owners of $v'$, namely $K_h(own_{h'}(v') \And  own_{h''}(v') \And (h' \ne h'')) \in \calK$, for some $h', h'' \in \calH$. 
    \item An agent $h \in \calH$ knows that $v'$ is duplicated if $h$ knows  that an agent $h' \in \calH$ is the owner of both $v', v'' \in V$, namely $K_h own_{h'}(v'), K_h own_{h'}  (v'') \in \calK$ and $v' \ne v''$.
\end{itemize}

Bearing this in mind, we can formalize the notions defined above:  
\begin{enumerate}
    \item $compromised(v) \Longleftrightarrow \exists h\exists h'  (h \ne h' \And own_{h}(v) \And  own_{h'}(v))$
    
    \item $duplicates(v,v') \Longleftrightarrow \exists h (own_{h}(v) \And own_{h}(v'))$
    
    
    \item $genuine (v) \Longleftrightarrow \neg compromised(v) \And \neg \exists v' duplicates(v,v')$
    
    \item $corrupt(v) \Longleftrightarrow  \neg genuine (v)
     \Longleftrightarrow compromised(v) \lor \exists v' duplicates(v,v')$
    
\end{enumerate}


Note that the abbreviated form of the definitions above uses no agent names, only global identifiers. Using them, we can now define the notion of reporting a sybil:
\begin{definition}[Reporting a Sybil]
An agent $h \in \calH$ \emph{reports an identity $v'$ as a sybil} if $C_h^v compromised(v') \in \calC$ or $C_h^v duplicates(v',v'')\in \calC$ for some  $v'' \ne v' \in V$. 
\qqed \end{definition}
Our intention is that as soon as an honest agent knows that a certain global identity is a sybil, it would report it.
 

%The report should include evidence establishing such knowledge.  The nature of the evidence is not part of the formal epistemic system, and may change as technology advances; e.g., it may include DNA snippets, iris scans, gate signatures, etc..  For example, and using present-day technology, a report of duplicate identifiers $v \ne v'$  may contain two selfie videos of the same person, in one the person claims, in its own voice, to own $v$ and the video being signed by the secret key of $v$, the other claiming to own $v'$ and signed by the secret key of $v'$. A report of a compromised identity $v$ may contain two selfie videos of two different people, each claiming to own $v$ and signed by the secret key of $v$.  


\begin{definition}[Reported Sybils]
Let $V$ be the set of global identifiers and $S \subset V$ the set of sybil identifiers in $V$.  The sybils $S = S_R \uplus S_U$ are divided into two disjoint subsets, the  \emph{reported sybils} $S_R$ and  the \emph{unreported sybils} $S_U$, where 
$$
S_R =  \{v \in S ~|~  \textrm{$\calC$ has a report that $v$ a sybil} \}
$$
\qqed \end{definition}


The following definition aims to formalize the notion that honest people know only reported sybils, with the rationale that an honest agent would report that an identity is a sybil as soon as it knows it to be one. 

\begin{definition}[Honest and Corrupt Genuine Global Identifiers]
Let $V=V_R \uplus V_U$ be a set of global identifiers.
An agent $h \in \calH$ is \emph{honest} if every  $v'$ that $h$ knows to be a sybil is reported as such, $v' \in S_R$, and
\emph{corrupt} otherwise, namely if $h$ knows that some $v'$ is a sybil and $v'$ is unreported, $v' \in S_U$.

A genuine global identity is \emph{honest} if its sole owner is honest and \emph{corrupt} otherwise. 
\qqed \end{definition}


%\begin{definition}[Coherent Identifier]
%A global identity $v \in V$ is  \emph{coherent} if there is an agent $h \in V$ such that for every global identifiers $v' \in V$ with owner $h' \in \calH$ and a trust edges $ kp(v' \rightarrow v) \in E$, if $h'$ knows that $x \in \calH$ owns $v$ then $x = h$.  In such a case $h$ is called the \emph{known owner of} $v$.  Otherwise $v$ is \emph{incoherent}.
%\qqed \end{definition}
%In other words, a global identity $v$ is incoherent if there are two agents that own global identifiers that trust $v$, yet know two different owners of $v$.

An agent $h$ with genuine global identity $v$ is \emph{prudent} 
if it knows all the mutual sureties of its friends; which means also that it knows all the friends of its friends.
\begin{definition}[Prudence]
Let $G=(V,E)$ be a surety graph. An agent $h \in \calH$ with genuine global identity $v \in V$ is \emph{prudent} with respect $G$ if  $(v, v'), (v', v'') \in E$ with witness $h',h'' \in \calH$ for $v',v''$, respectively, implies that $K_h S_{h',h''}(v',v'') \in \calK$, for all $v', v'' \in V$.
\qqed \end{definition}

Our goal is to bound the fraction of sybils in a valid trust graph, given that all honest agents are prudent and that the fraction of corrupt agents in the population is sufficiently small.  Additional assumptions we will need are that the trust graph is valid and has sufficient conductance. 


\begin{observation}
Consider a surety graph $G=(V,E)$ and a prudent agent $v \in V$.  If $(v, v') \in E$ and $v'$ is compromised in $G$, then $v$ knows that $v'$ is compromised. 
\end{observation}
\begin{proof}
Similar to the proof of Observation \ref{observation:-compromised-in-graph}
\end{proof}


Let $G=(V,E)$ be an undirected graph.  Recall that
a the distance $d(v,v)$ between two vertices $v,v' \in V$ is the minimal number of edges in $E$ in any path connecting $v$ and $v'$. The \emph{ball} of radius $r$ around $v \in V$ contains all vertices $\{v ~|~ d(v,v') \le r\}$.

\begin{lemma}
Consider a surety graph $G=(V,E)$ and a prudent agent $v \in V$.  If all honest neighbours of $v$ in $G$ are also prudent, and the ball of radius 2 of $v$ in $G$ has duplicates $v', v'' \in V$ connected to $v$ via honest agents, if any, then $v$ knows that   $v', v''$ are duplicates.
\end{lemma}
\begin{proof}
There are three cases to consider
\end{proof}



\begin{definition}[Honest and Corrupt Identifiers]
A trust edge $v \rightarrow v' \in V$ is \emph{honest} 
if $v$ is a genuine global identity and its owner knows the owner of $v'$ and does not know that $v'$ is compromised or duplicated. A global identity $v \in V$ is \emph{honest} if every trust edge $v \rightarrow v' \in E$ is honest, \emph{corrupt} otherwise.
\qqed \end{definition}


\subsection{Suspending, Recovering, and Updating Identifiers}

To suspend/abolish/recover/update identifiers in case they are uncovered as sybils, lost, stolen or obsolete, the repository also maintains an \emph{update list} of pairs of the form (identity, status). The first element is an identity. The second element could be the new status, e.g. suspended or abolished, or a new identity that supplants this identity.

A lost or stolen identity $p=K_P^t$ is replaced by creating a new identity $p'=(K'_P^{t'})$, in which the keys and time-stamp are new, and storing in the update list the pair $(K_P^t,K'_P^{t'})$.  How updates to the update list are authorized is discussed below.


\subsection{Detecting Duplicate Identifiers}

We employ  detect duplicate identifiers based on \emph{citizens reports}:  When a person sees that another person employs two identifiers, these identifiers can be reported.  This may be sufficient, assuming:
\begin{itemize}
    \item Only a few people will attempt to create duplicate identifiers.
    \item Among those who do, only a few can maintain two identifiers for a long period of time, without another person eventually spotting that.
    \item Effective punishment for creators of duplicate identifiers, and effective compensation for those who detect and report them, may create a positive feedback loop that decreases the prevalence of duplicate identifiers.
    \item We can tolerate a reasonable (say single-digit) penetration of sybil identifiers\cite{srsc}.
\end{itemize}


\subsection{Recovering Lost or Stolen Global Identifiers}

To address the problem of lost or stolen (private key of an) identity we suggest the following mechanism:

For each identity $p$, there is a ``superminority'', suspend($p$), of its trusted identifiers that are sufficient to declare that $p$ is suspended and a ``supermajority'', replace($p$) of its trusted identifiers that are needed to declare that $p$ is replaced by $p'$.  Formally, suspend($p$) and replace($p$) denote sets of subsets of the identifiers trusted by $p$, each of which is sufficient to effect the corresponding operation.  $p$ would specify explicitly the suspend and replace subsets of its trusted identifiers.

We envision that upon discovery by $h$, the rightful owner of $p$, that the private key of $p$ has been lost, stolen, or otherwise compromised, $p$ would judicially approach its trusted people and ask them to declare $p$ suspended.  Once a sufficient group of the identifiers trusted by $p$, a superset of an element of suspend($p$), declares that $p$ is suspended, this fact is recorded in the global identity ledger. Once $p$ has been suspended, $h$ would create a new identity $p'$ and ask all its trusted people to declare that $p$ is replaced by $p'$. Once a sufficient group of the identifiers trusted by $p$, a superset of an element of replace($p$), has declared so, the global identifiers ledger would record this update.

The suspension of an identity $p$ would entail the freezing of the cryptoassets of $p$, and the replacement of an identity $p$ by $p'$ would entail the transfer of these assets from $p$ to $p'$.  Hence, the suspend and replace subsets of trusted identifiers should be carefully chosen. Furthermore, emergency measures for blocking identity update in case there is probable cause to suspect that a group of identifiers has fallen victim to organized crime should be considered.





\end{document}


[To be rewritten]
An agent $h \in \calH$ may perform the following knowledge-creating operations:

\begin{enumerate}
    \item \textbf{Create a global identity:}  Create a new key-pair $(p,s)$, in which case $K_h  kp(p,s)$ is added to $\calK$.
    \item \textbf{Prove ownership of its global identity:}  Engage in a dialogue with an agent $h' \in \calH$ that causes $h'$ to know that $h$ owns $v$, in which case $K_{h'}\exists s K_h  kp(v,s)$ is added to $\calK$.
    \item \textbf{Compromise its global identity:}  Disclose\footnote{Of course such disclosure could be inadvertent, malicious, or under duress.} the key-pair $(v,s)$ of a global identity $v  \in V$ it owns  to an agent $h' \ne h \in \calH$, in which case $K_{h'}  kp(v,s)$ is added to $\calK$.
    
    \item \textbf{Make its knowledge common, judiciously:}  Add $C\exists x_1, \ldots \exists x_n X'$ to $\calK$, $n \ge 0$, provided $K_h X \in \calK$, where $X'$ is obtained from $X$ by consistently replacing constants $c_1,\ldots c_n$ by the variables $x_1, \ldots x_n$, thus making its personal knowledge $X$ common, while keeping the witnesses $c_1, \ldots c_n$ to $X$ private. 
    
    
%    \item \textbf{Prove honesty of edge:}  Engage in a dialogue with an agent $h' \in \calH$ that causes $h$ to know that an edge $v\rightarrow v''$ is decent edge. Formally, assume that $h'$ knows that $h''$ owns $v''$ ($K_{h'} K_{h''}  kp(v'',s)\in \calK$). In the end of the dialogue $h'$ should know that $h$ knows that $h''$ owns $v''$ ($K_{h} K_{h''}  kp(v'',s)\in \calK$), in which case $K_{h'} K_{h} K_{h''}  kp(v'',s)$ is added to $\calK$. 

\end{enumerate}
    

\end{document}
